On the Semantics of Intensionality and Intensional Recursion

Intensionality is a phenomenon that occurs in logic and computation. In the most general sense, a function is intensional if it operates at a level finer than (extensional) equality. This is a familiar setting for computer scientists, who often study different programs or processes that are interchangeable, i.e. extensionally equal, even though they are not implemented in the same way, so intensionally distinct. Concomitant with intensionality is the phenomenon of intensional recursion, which refers to the ability of a program to have access to its own code. In computability theory, intensional recursion is enabled by Kleene's Second Recursion Theorem. This thesis is concerned with the crafting of a logical toolkit through which these phenomena can be studied. Our main contribution is a framework in which mathematical and computational constructions can be considered either extensionally, i.e. as abstract values, or intensionally, i.e. as fine-grained descriptions of their construction. Once this is achieved, it may be used to analyse intensional recursion.

==> Makefile <==
TEX = pdflatex -file-line-error

main : main.tex \
         abstract.tex dedication.tex intro.tex
	$(TEX) -draftmode main
	# bibtex main
	# $(TEX) -draftmode main
	$(TEX) main

all:
	cd srtht; make
	make main

clean :
	rm -f packages/modal-macros.aux
	rm -f *.aux
	rm -f *.log
	rm -f *.ptb
	rm -f *.blg
	rm -f *.lof
	rm -f *.toc
	rm -f *.out
	rm -f main.pdf


==> agda/Makefile <==
agda :
	agda --include-path=. \
	     --include-path=/usr/share/Agda-stdlib \
	     --latex Basics.lagda
	agda --include-path=. \
	     --include-path=/usr/share/Agda-stdlib \
	     --latex iPCF.lagda
	agda --include-path=. \
	     --include-path=/usr/share/Agda-stdlib \
	     --latex iPCF2.lagda

clean :
	rm -f *.agdai
	rm -f *.agda~
	rm -f *.lagda~


==> asm.tex <==
In this \kwhat{} we study our central example of an exposure,
which hails from realizability.

The basic objects in realizability are \emph{assemblies}: an
assembly is a set of which every element is associated with a
\emph{set of realizers}. The elements of the set can be thought of
as the elements of an \emph{abstract datatype}, whereas the set of
realizers of each element contains its multiple
\emph{machine-level representations}. For example, realizers can
range over the natural numbers; then, taking functions between
assemblies which can be `tracked' on the level of realizers by
partial recursive functions yields a category where `everything is
computable.'

In practice, the generalization from natural numbers to an
arbitrary \emph{partial combinatory algebra (PCA)} is made. A PCA
is an untyped `universe' corresponding to some notion of
computability or realizability. There are easy tricks with which
one may encode various common `first-order' datatypes (such as
booleans, integers, etc.) in a PCA.\footnote{Most of these tricks
have their origins in untyped $\lambda$-calculus, and hence can
also be found in \cite{Barendregt1984}.} Moreover, it is easy to
show that, up to a simple representation of integers, one may
represent all partial recursive functions in a PCA. We recap the
basics of PCAs, but detailed discussions may be found in
\citep{Beeson1985, Longley1995, Longley1997, VanOosten2008}.

Once a PCA---and hence a notion of computability---is fixed, it is
quite clear how to define a P-category. Objects are assemblies,
and morphisms are functions which are `computable' on the level of
realizers. The arrows are pairs $(f, r)$ where $f$ is a function
on the underlying set of each assembly, and $r$ is an element of
the PCA that tracks the function $f$. Two arrows are related if
and only if they define the same function on the underlying sets.
Finally, to define an endoexposure all we need to do is display
the effect of each tracking element $r$ on the realizers.

\psubsection{Partial Combinatory Algebras}

The definition of a PCA is deceptively simple:

\begin{defn}
  A \emph{partial combinatory algebra (PCA)} $(A, \cdot)$ consists
  of a set $A$ and a partial binary operation $\cdot : A \times A
  \parfunc A$ such that there exist $\mb{K}, \mb{S} \in A$ with
  the properties that \[
    \mb{K} \cdot x\downarrow, 
      \quad
    \mb{K} \cdot x \cdot y \simeq y,
      \quad
    \mb{S} \cdot x \cdot y\downarrow,
      \quad
    \mb{S} \cdot x \cdot y \cdot z \simeq x \cdot z \cdot (y \cdot z)
  \] for all $x, y, z \in A$.
\end{defn}

The paradigmatic example comes from ordinary computability theory,
as presented by e.g. \cite{Cutland1980, Odifreddi1992,
Rogers1987}. It is not very difficult to use the S-m-n theorem to
cook up indices that behave like $\mb{S}$ and $\mb{K}$, to the
effect that
\begin{thm}[Kleene's First Model]
  The applicative structure \[
    K_1 = (\mathbb{N},\ \cdot\ )
  \] where \[
    x \cdot y \simeq \phi_x(y)
  \] is a partial combinatory algebra.
\end{thm} 

\psubsubsection{Combinatory Completeness}

We can also use standard tricks from untyped $\lambda$-calculus
and combinatory logic to greatly simplify calculations in a PCA.
Nevertheless, not all common rules of the untyped
$\lambda$-calculus do not hold in general, so we should be
cautious. This particular development is due to
\cite{Longley1995}.

\begin{defn} Let $V$ be an infinite set of variables. The set
$\mathcal{E}(A)$ of \emph{terms} or \emph{formal expressions} over a
PCA $(A, \cdot)$ is defined as the least set that satisfies the
following conditions: \[
  A \subseteq \mathcal{E}(A), \quad V \subseteq \mathcal{E}(A)
\] \[
  s \in \mathcal{E}(A) \;\; \& \;\; t \in \mathcal{E}(A) \quad
  \Longrightarrow \quad (s \cdot t) \in \mathcal{E}(A)
\] \end{defn} Conventionally, we will use $e, s, t, u, v, \dots$
as metavariables ranging over $\mathcal{E}(A)$, and we will
write $s[t/x]$ for the formal expression obtained by
substituting $t \in \mathcal{E}(A)$ for every occurrence of the
variable $x$ in the formal expression $s \in \mathcal{E}(A)$, in
the standard way. 

Next, a formal expression is \emph{closed} if it contains no
variables. Write $\fv(e)$ for the set of free variables of
expression $e \in \mathcal{E}(A)$. Also, we now write
$e\downarrow$ (``$e$ denotes'') for a closed formal expression
to mean that, if the formal expression is interpreted as an
actual algebraic expression in the standard way, it actually
denotes an element. This implies that all subexpressions also
denote: if $s \cdot t\downarrow$, then $s\downarrow$ and
$t\downarrow$. Otherwise, we write $e\uparrow$ to mean that, if
$e$ is interpreted as an algebraic expression, partiality kicks
in and the expression does not denote an element in the PCA.

We also notationally  distinguish two equalities: the strict
equality, $s = t$, where both $s\downarrow$ and $t\downarrow$
and they denote the same element; and the Kleene equality, $s
\simeq t$, which holds when $s$ and $t$ are both undefined,
or both defined and denote the same element.

Finally, the above notions are straightforwardly extended to
open terms, by substituting for all variables: let the variables
of $s, t \in \mathcal{E}(A)$ be amongst $x_1, \dots, x_n$; then,
for example \begin{align*}
  &e\downarrow \quad &\text{just if} \quad
    &\forall a_1, \dots, a_n \in A. \;
    e[\vec{a}/\vec{x}]\downarrow \\
  &s \simeq t \quad &\text{just if} \quad
    &\forall a_1, \dots, a_n \in A. \;
    s[\vec{a}/\vec{x}] \simeq t[\vec{a}/\vec{x}]
\end{align*} for the obvious generalisation to simultaneous
substitution. We can now $\lambda$-abstract:
\begin{lem}[Combinatory Completeness] Let $(A, \cdot)$ be a PCA.
For any $e \in \mathcal{E}(A)$, there exists a formal expression
$\lambda^\ast x. e \in \mathcal{E}(A)$, where 
$\fv(\lambda^\ast x. e) = \fv(e) - \{x\}$, such that \[
  \lambda^\ast x. e\downarrow
\] and \[
  (\lambda^\ast x. e)a \simeq e[a/x]
\] for all $a \in A$. \end{lem} \begin{proof} Define
\begin{align*} \lambda^\ast x. x &= \mb{S} \cdot \mb{K} \cdot \mb{K} & \\
  \lambda^\ast x. t &= \mb{K} \cdot t &\text{ if $t \in A \cup V$ and
  $t \not\equiv x$} \\
  \lambda^\ast x. s \cdot t &= \mb{S} \cdot (\lambda^\ast x. s)
  \cdot (\lambda^\ast x. t) & \end{align*} Then $\lambda^\ast x.
  e\downarrow$ by the
definedness conditions for $\mb{S}$ and $\mb{K}$. The rest
follows by induction. \end{proof} Let us be pedantic and reiterate
the warnings: Kleene equality is \emph{not} respected by the
$\lambda^\ast x$ operation on terms, and the obvious $\beta$-rules
do not hold---observe that the operand above has to be a constant!
Longley carefully develops correct $\beta$-rules for this language
of terms in \citep[1.1.2]{Longley1995}.

\psubsubsection{Some common encodings}

We will need the following combinators:
\begin{align*}
  \mathbf{I} &\myeq \mathbf{S}\mathbf{K}\mathbf{K} \\
  \mathbf{B} &\myeq \lambda^\ast f. \lambda^\ast g. \lambda^\ast x. f (g x)
\end{align*}

It is easy to define selection and pairs. Let \begin{align*}
  \textsf{true}  &\myeq \lambda^\ast a b . a \\
  \textsf{false} &\myeq \lambda^\ast a b . b \\
  \textsf{if}    &\myeq \lambda^\ast xyz. xyz \\
  \textsf{pair}  &\myeq \lambda^\ast xyz. zxy \\
  \textsf{fst}   &\myeq \lambda^\ast p. p(\textsf{true})\\
  \textsf{snd}   &\myeq \lambda^\ast p. p(\textsf{false})
\end{align*} We always have $\textsf{if}\ x\ y \downarrow$,
and $\textsf{pair}\ x\ y \downarrow$. Further, the following
equalities hold: \begin{align*}
  \textsf{fst}\ (\textsf{pair}\ x y) &= x \\
  \textsf{snd}\ (\textsf{pair}\ x y) &= y \\
  \textsf{if}\ \textsf{true}\ y z &= y \\
  \textsf{if}\ \textsf{false}\ y z &= z
\end{align*}

It is not much harder to encode numbers, and, like
\citep{Longley1995, Longley1997}, we use a trick due to Curry. Let
\begin{align*}
  \overline{0} &= \mathbf{I} \\
  \overline{n+1} &= \textsf{pair}\ \textsf{false}\ \overline{n}
\end{align*} Then we may let $\textsf{succ} = \lambda^\ast x.
\textsf{pair}\ \textsf{false}\ x$, so that $\textsf{succ}\
\overline{n} = \overline{n+1}$. 

To check if a number is zero, use $\textsf{iszero}\ \myeq
\textsf{fst}$ so that \[
  \textsf{iszero}\ \overline{0} = \mathbf{I}
  (\textsf{true}) = \textsf{true}
\] whereas \[
  \textsf{iszero}\ \overline{n+1} = \textsf{fst}\ (\textsf{pair}\
  \textsf{false}\ \overline{n}) = \textsf{false}
\] Finally, we can define the predecessor function by \[
  \textsf{pred} \myeq \lambda^\ast x. \textsf{if}\
  (\textsf{iszero}\ tx)\ \overline{0}\ (\textsf{snd}\ x)
\]

\psubsection{Assemblies and Modest Sets}

\begin{defn} An \emph{assembly} $X$ on $A$ consists of a set
$\left\lvert X \right\rvert$ and, for each $x \in \left\lvert X
\right\rvert$, a non-empty subset $\left\|x\right\|_X$ of $A$.  If
$a \in \left\|x\right\|_X$, we say that \emph{$a$ realizes $x$}.

\end{defn}

\begin{defn} For two assemblies $X$ and $Y$, a function $f :
\bars{X} \rightarrow \bars{Y}$ is said to be \emph{tracked by $r
\in A$} just if, for all $x \in \bars{X}$ and $a
\in \dbars{x}_X$, we have \[
  r \cdot a \downarrow
    \quad \text{and} \quad 
  r \cdot a \in \dbars{f(x)}_Y
\] \end{defn}

\begin{defn} An assembly $X$ on $A$ is a \emph{modest set} just if no
element of $A$ realizes two elements of $\bars{X}$. That is, \[
  x \neq x' \quad \Longrightarrow \quad \dbars{x}_X \cap
  \dbars{x'}_X = \emptyset
\] \end{defn}

\noindent It is not hard to see that, for each PCA $A$, we can
define a category $\mathbf{Asm}(A)$, with objects 
all assemblies $X$ on $A$, and morphisms $f : X \rightarrow Y$
being functions $f : \bars{X} \rightarrow \bars{Y}$ that are
tracked by some $r \in A$. In fact,

\begin{thm} 
  Assemblies and trackable morphisms between them form a
  category $\mathbf{Asm}(A)$ that is cartesian closed, has
  coproducts, as well as a natural numbers object.
\end{thm}

It is not clear who originated the (admittedly very intuitive)
definition of $\mathbf{Asm}(A)$. \cite{Longo1991} refer to it as
the category of $\omega$-sets, and so does \cite{Jacobs1999}.  For
more detailed constructions, see \citep{Longley1995} or
\citep{Longley1997}. 

A special subcategory of the above is of particular interest:

\begin{thm}
  The full subcategory of $\mathbf{Asm}(A)$ consisting only of
  objects which are modest sets, which we denote by
  $\mathbf{Mod}(A)$, inherits the cartesian closed, coproduct, and
  natural number object structure from the category of assemblies.
\end{thm}

The category of modest sets---or its equivalent presentation in
terms of PERs on the PCA $A$---seems to have originated
independently in the work of \cite{Scott1976} on domain theory,
and \cite{Girard1972} on the semantics of System F. Accessible
presentations may be found in \cite{Mitchell1996} or
\cite{Crole1993}.

\psubsection{Passing to a P-category}

The lack of intensionality in the category $\mathbf{Asm}(A)$ is
perhaps more obvious than anywhere else. To elevate a function $f
: \bars{X} \rightarrow \bars{Y}$ to a morphism $f : X \rightarrow
Y$, we only require that \emph{there exists} a $r \in A$: as soon
as this is witnessed, we forget the witness entirely. For all the
reasons stated in \S\ref{sec:catint} we have to pass to
P-categories to mend this.

The P-category of assemblies on $A$, written $\mathfrak{Asm}(A)$,
is defined as follows. Its objects are once more all assemblies
$X$ on $A$. Given assemblies $X$ and $Y$, the P-set
$\mathfrak{Asm}(X, Y)$ is defined by having underlying set \[
  \bars{\mathfrak{Asm}(X, Y)} \myeq
    \setcomp{ (f : \bars{X} \rightarrow \bars{Y}, r \in A) }
            { r \text{ tracks } f}
\] and \[
  (f, r) \sim_{\mathfrak{Asm}(X, Y)} (g, s)
    \quad\text{just if}\quad
  f = g
\] For $(f, r) : X \rightarrow Y$ and $(g, s) : Y \rightarrow Z$,
we define composition by \[
  (g, s) \circ (f, r) \myeq (g \circ f, \mb{B} \cdot s \cdot r)
\] Notice that for any $x \in \bars{X}$, $a \in \dbars{x}_X$
implies $p \cdot a \in \dbars{f(x)}_Y$, which implies $q \cdot (p
\cdot a) \in \dbars{g(f(x))}_Z$, and as $\mb{B} \cdot q \cdot p
\cdot a \simeq q \cdot (p \cdot a)$ it follows that $(g \circ f,
\mb{B} \cdot p \cdot q)$ is an arrow $X \rightarrow Z$. It is easy
to see that this is a P-function, for composition of set-theoretic
functions is associative. 

We define the identity $id_X : X \rightarrow X$ to simply be
$(id_{\bars{X}}, \mathbf{I})$, and it is evident that $id_Y \circ
f \sim f \sim f \circ id_X$ for any $f : X \rightarrow Y$.

\psubsubsection{Finite Products}

It is not hard to show that 

\begin{lem} 
  The category $\mathfrak{Asm}(A)$ has binary products.
\end{lem}

\begin{proof}
  The construction essentially follows the underlying
  structure of products in the category of sets, but augments it
  with tracking elements. For assemblies $X$ and $Y$, we define \[
    \bars{X \times Y} := \bars{X} \times \bars{Y},
      \qquad
    \dbars{(x, y)}_{X \times Y} := \setcomp{ \textsf{pair}\,a\ b }
    { a \in \dbars{x}_{X}, b \in \dbars{y}_Y }
  \] The projections are the following 1-cells:
  \begin{align*}
    \pi_1  &\myeq (\pi_1 : \bars{X} \times \bars{Y} \rightarrow \bars{X},
      \textsf{fst}) \\
    \pi_2 &\myeq (\pi_2 : \bars{X} \times \bars{Y} \rightarrow \bars{Y},
      \textsf{snd})
  \end{align*} Define the P-function $\langle -, -\rangle$ by \[
    \left\langle (f, r), (g, s) \right\rangle 
      \myeq \left(\langle f, g \rangle, \lambda^\ast c.\
    \textsf{pair}\ (r c) (s c)\right)
  \] It is easy to see that this is a P-function.
  We compute that \[
    \pi_1 \circ \langle (f, r), (g, s) \rangle = 
      (f,
	\mathbf{B} \cdot \mathsf{fst}
	  \cdot (\lambda^\ast c.\, \mathsf{pair}\,(r c)\ (s c)))
    \sim (f, r)
  \] and similarly for the other two equations.
\end{proof}

\begin{lem}
  The P-category $\mathfrak{Asm}(A)$ has a terminal object.
\end{lem}

\begin{proof}
  Define $\mathbf{1} \in \mathfrak{Asm}(A)$ by \[
    \bars{\mathbf{1}} := \{\ast\},
      \qquad
    \dbars{\ast}_\mathbf{1} := \{ \overline{0} \}
  \] and, for $A \in \mathfrak{Asm}(A)$, let ${!}_A := (a \mapsto
  \ast, \mathbf{K} \cdot \overline{0}) : A \rightarrow
  \mathbf{1}$.
\end{proof}

Hence,

\begin{thm}
  $\mathfrak{Asm}(A)$ has finite products.
\end{thm}

\psubsubsection{Exponentials}

Given assemblies $X$ and $Y$, we define \[
  \bars{Y^X} := \setcomp{ f }{ (f, r) : X \rightarrow Y }, \qquad
  \dbars{f}_{Y^X} := \setcomp{ r }{ r \text{ tracks } f }
\] Let \[
  \textsf{ev}_{X, Y} := ((f, x) \mapsto f(x), \lambda^\ast p.\,
  (\textsf{fst } p) (\textsf{snd } p)) : Y^X \times X \rightarrow
  Y
\] Define a P-function \[
  \lambda_C : 
    \mathfrak{Asm}(A)(C \times X, Y)
      \rightarrow
    \mathfrak{Asm}(A)(C, Y^X)
\] by \[
  (f, r) \mapsto (z \mapsto (x \mapsto f(z, x)), \lambda^\ast c.\,
  \lambda^\ast a.\, r (\textsf{pair } c\, a))
\] It is again easy to see that this is a P-function, and one can
verify that this is the exponential. Therefore,

\begin{thm}
  The bicategory $\mathfrak{Asm}(A)$ is cartesian closed.
\end{thm}

\psubsection{The Exposure}

\begin{thm} There is an exposure, \[
  \Box : \mathfrak{Asm}(A) \looparrowright \mathfrak{Asm}(A)
\] for any PCA $A$. \end{thm}
\begin{proof}
  For an assembly $X \in \mathfrak{Asm}(A)$, let $\Box
  X$ be the assembly defined by \begin{align*}
    \bars{\Box X} &\myeq \setcomp{ (x, a) }
      { x \in \bars{X}, a \in \dbars{x}_A} \\
    \dbars{(x, a)}_{\Box X} &\myeq \{\ a\ \}
  \end{align*} Given $(f, r) : X \rightarrow Y$, we define $
    \Box(f, r) = (f_r, r) : \Box X \rightarrow \Box Y
  $ where \begin{align*}
    f_r : \bars{\Box X} &\rightarrow \bars{\Box Y} \\
	     (x, a)        &\longmapsto (f(x), r \cdot a)
  \end{align*} Each element $(x, a) \in \bars{\Box X}$ has a unique
  realizer, $a$. As $a \in \dbars{x}_X$, and $f$ is tracked by $r$,
  we see that $r \cdot a \downarrow$ and $r \cdot a \in \dbars{f(x)}_{\Box
  Y}$, so that $(f(x), r \cdot a) \in \bars{\Box Y}$. It follows
  that $r$ tracks $f_r$ and so $(f_r, r)$ is an arrow $\Box X
  \rightarrow \Box Y$.

  To prove that $\Box$ preserves composites, observe that for
  arrows $(f, r) : A \rightarrow B$ and $(g, s) : B \rightarrow C$,
  we have \[
    (x, a)
      \overset{f_r}{\longmapsto}
    (f(x), r \cdot a)
      \overset{g_s}{\longmapsto}
    \left(g(f(x)), s \cdot (r \cdot a)\right)
  \] and as $\mathbf{B} \cdot s \cdot r \cdot a \simeq s \cdot (r
  \cdot a)$, we have \[
    g_s \circ f_r = (g \circ f)_{\mathbf{B} \cdot s \cdot r}
  \] which is of course tracked by $\mathbf{B} \cdot s \cdot r$.
  Hence $\Box(g \circ f) \sim \Box g \circ \Box f$. Regarding
  identities, notice that if $id_X : X \rightarrow X$ is the
  identity arrow, then \[
    (x, a) \overset{\left(id_X\right)_{\mathbf{I}}}
      \longmapsto 
    (x, \mathbf{I} \cdot a)
  \] and as $\mathbf{I} \cdot a \simeq a$, the latter is equal to
  $(x, a)$, so $\left(id_X\right)_\mathbf{I} \sim id_{\Box X}$.
  Hence $\Box id_X \sim id_{\Box X}$.

  Finally, we need to show that intensional equality implies
  extensional equality. Suppose $\Box (f, r) \Box (g, s)$. That is
  equivalent to $f_r = g_s$, which in turn gives us both $f = g$ and
  also $r \cdot a \simeq s \cdot a$ for all $a \in \dbars{x}_X$. The
  first implies $(f, r) \sim (g, s)$.
\end{proof}

\psubsection{Intensional Equality}

When showing that $\Box$ is an exposure, we inadvertently
characterised intensional equality up to $\Box$:

\begin{lem}
  $(f, r) \approx (g, s) : X \rightarrow Y$ precisely when $f_r =
  g_s$, i.e. \[
  f = g \quad \text{and} \quad 
    \forall x \in \bars{X}.\
    \forall a \in \dbars{x}_X.\
      r \cdot a \simeq s \cdot a
  \]
\end{lem}

\begin{defn}
  An assembly $X$ has \emph{unique realizers} just if
  $\dbars{x}_X$ is a singleton, for each $x \in \bars{X}$.
\end{defn}

\begin{thm}
  The univalent objects of $\mathfrak{Asm}(A)$ are precisely those
  which have unique realizers.
\end{thm}
\begin{proof}
  Suppose $X$ is univalent. To each realizer $a \in
  \dbars{x}_X$, there corresponds an arrow \[
    \hat{x}_a \myeq (\ast \mapsto x, \lambda^\ast c. a)
      : \mathbf{1} \rightarrow X
  \] But if $a, b \in \dbars{x}_X$, then $\hat{x}_a \sim
  \hat{x}_b$, as they share the same function component $(\ast
  \mapsto x)$. As $X$ is univalent, it follows that $\hat{x}_a
  \approx \hat{x}_b$, so \[
    a \simeq (\lambda^\ast c. a) \cdot \overline{0} 
      \simeq (\lambda^\ast c. b) \cdot \overline{0}
      \simeq b
  \]

  Conversely, suppose $X$ has unique realizers. For any two
  extensionally equal arrows $(f, r), (f, s) : Y \rightarrow
  X$, it is not very hard to see that $f_r = f_s$: we have that
  $\pi_1(f_r(y, b)) = f(y) = \pi_1(f_s(y, b))$ for any $b \in
  \dbars{y}_Y$. Thus, as $f(y)$ is uniquely realized by only one
  $a$, their second components are equal too, and $(f, r) \approx
  (f, s)$.
\end{proof}

\psubsection{Cartesianness}

It so happens that projections behave as expected under exposures,
i.e. 

\begin{thm}
  $\Box : \mathfrak{Asm}(A) \looparrowright \mathfrak{Asm}(A)$ is
  a cartesian exposure.
\end{thm}

\noindent Recall that $\pi_1 \circ \langle (f, r), (g, s) \rangle
= (f, d)$, where \[
  d \myeq \mathbf{B} \cdot \mathsf{fst} \cdot (\lambda^\ast c.\,
    \mathsf{pair}\ (r c) (s c))
\] so that the function component of $\Box (\pi_1 \circ \langle
(f, r), (g, s) \rangle)$ is $f_d(z, c) = (f(z), d \cdot c)$. We
compute that $d \cdot c$ is equal to \begin{align*}
  &\mathbf{B} \cdot \mathsf{fst} \cdot (\lambda^\ast c.\,
        \mathsf{pair}\ (r c) (s c)) \cdot c \\
  =\ &\mathsf{fst} \cdot ((\lambda^\ast c.\,
          \mathsf{pair}\ (r c) (s c)) \cdot c) \\
  =\ &\mathsf{fst} \cdot (\mathsf{pair}\ (r c) (s c)) \\
  =\ &r \cdot c
\end{align*} That is, \[
  f_d = f_r
\] and hence $\Box(\pi_1 \circ \langle
(f, r), (g, s) \rangle) \sim \Box f$, and similarly for the other
projection.

For the third equation, it is easy to calculate that, for any
arrow $h : C \rightarrow X \times Y$, the function component of
$\Box\langle \pi_1 \circ (h, r), \pi_2 \circ (h, r) \rangle$ is
$h_s$, where \[
  s = \lambda^\ast c.\,\textsf{pair}\ (\mathbf{B} \cdot
  \mathsf{fst} \cdot r \cdot c)\,(\mathbf{B} \cdot \mathsf{snd}
  \cdot r \cdot c)
\] We proceed by calculating that \[
  s \cdot c
  = \textsf{pair}\ 
      (\mathbf{B} \cdot \mathsf{fst} \cdot r \cdot c)\
      (\mathbf{B} \cdot \mathsf{snd} \cdot r \cdot c)
  = \textsf{pair}\
      (\textsf{fst}\ (r \cdot c))\
      (\textsf{snd}\ (r \cdot c))
\] so that \[
  h_s(z, c) =
    (h(z),
      \textsf{pair}\ (\textsf{fst}\ (r c))\ (\textsf{snd}\ (r c)))
\] The argument would now be complete were our pairing surjective,
but this is not so in general PCAs. However, we can make use of
what we know regarding the structure of $r$. It is
known that $r$ tracks $h : C \rightarrow X \times Y$; it follows
that, if we let $h(z) = (x, y)$ with $x \in \bars{X}$ and $y \in
\bars{Y}$, then, whenever $c \in \dbars{z}_C$, \[
  r \cdot c = \textsf{pair}\ a\ b
\] for some $a \in \dbars{x}_X$ and $b \in \dbars{y}_Y$. Therefore
$s \cdot c = \textsf{pair}\ a\ b$ and thus  $h_s = h_r$, where $r$
was the original tracking element of $(h, r)$. We have finally
obtained that \[
  \Box\langle \pi_1 \circ (h, r), \pi_2 \circ (h, r) \rangle 
    \sim \Box (h, r)
\] and hence the exposure is cartesian.


\psubsection{Preservation of Products}

Define \[
  m_0 \myeq (\ast \mapsto (\ast, \overline{0}), \mathbf{I})
    : \mathbf{1} \rightarrow \Box \mathbf{1}
\] which maps the unique element of $\mathbf{1}$ to the pair of
itself and its unique realizer, and is realized by the identity
combinator. This is a P-isomorphism with inverse \[
  {!}_{\Box \mathbf{1}} \myeq
    ((\ast, \overline{0}) \mapsto \ast, \mathbf{I})
      : \Box \mathbf{1} \rightarrow \mathbf{1}
\] Also, define $m_{A, B} : \Box A \times \Box B \rightarrow \Box
(A \times B)$ by $m_{A, B} \myeq (w_{A, B}, \mathbf{I})$, where
\begin{align*}
  w_{A, B} : &\bars{\Box A} \times \bars{\Box B} \rightarrow \bars{\Box (A \times B)}\\
             &((x, a), (y, b)) \mapsto ((x, y), \textsf{pair}\,a\,b)
\end{align*} The only realizer for the pair $((x, a), (y, b))$ is
$\textsf{pair}\,a\, b$, so the identity combinator tracks
$w_{A, B}$. Then $\langle \Box\pi_1, \Box\pi_2 \rangle : \Box (A
\times B) \rightarrow \Box A \times \Box B$ is equal to
$(v_{A, B}, \mathbf{I})$, where \begin{align*}
  v_{A, B} : &\bars{\Box (A \times B)} \rightarrow \bars{\Box A} \times \bars{\Box B} \\
	     &((x, y), r) 
	      \mapsto ((x, \textsf{fst} \cdot r),
	               (y, \textsf{snd} \cdot r))
\end{align*} and it is trivial to see that it is an inverse to
$m_{A, B}$. Hence

\begin{thm}
  The exposure $\Box : \mathfrak{Asm}(A) \expo{}
  \mathfrak{Asm}(A)$ is product-preserving.
\end{thm}

\psubsection{Comonadicity}

\begin{lem}
  There exists a natural transformation of exposures, \[
    \epsilon : \Box \natexp \mathsf{Id}_{\mathfrak{Asm}(A)}
  \]
\end{lem}

\begin{proof}
  Define $\epsilon_X = (u_X, \mathbf{I})$, where \begin{align*}
    u_X : \bars{\Box X} &\rightarrow \bars{X} \\
	  (x, a)        &\longmapsto x
  \end{align*} If $b \in \dbars{(x, a)}_{\Box X} = \{ a \} $, then $b = a$ and
  $\mathbf{I} \cdot b \simeq b = a \in \dbars{x}_X$, so $u_X$ is
  indeed tracked by $\mathbf{I}$. To show naturality for a given
  1-cell $(f, r) : X \rightarrow Y$, we chase around the diagram: \[
    \begin{tikzcd}
      (x, a)
	\arrow[r, mapsto, "f_r"]
	\arrow[d, mapsto, swap, "u_X"]
      & (f(x), r \cdot a)
	\arrow[d, mapsto, "u_Y"] \\
      x
	\arrow[r, mapsto, swap, "f"]
      & f(x)
    \end{tikzcd}
  \] Hence $u_Y \circ f_r = f \circ u_X$, so the square commutes up
  to $\sim$.  Bear in mind that the tracking
  element along one composite is $\mathbf{B} \cdot r \cdot
  \mathbf{I}$, whereas along the other composite it is $\mathbf{B}
  \cdot \mathbf{I} \cdot r$.
\end{proof}

Let us now investigate the structure of $\Box^2 X$, for any
assembly $X$. For each $(x, a) \in \bars{\Box X}$, we have that
$\dbars{(x, a)}_{\Box X} = \{ a \}$. Thus, we can infer that \[
  \bars{\Box^2 X} = \setcomp{((x, a), a)}{a \in \dbars{x}_X}
\] and that, for any $(f, r) : X \rightarrow Y$, \begin{align*}
  v_X : \bars{\Box^2 X} &\longrightarrow \bars{\Box^2 y} \\
        ((x, a), a)        &\longmapsto ((f(x), r \cdot a), r \cdot a)
\end{align*}

\begin{lem}
  There exists a natural transformation of exposures, \[
    \delta : \Box \natexp{} \Box^2
  \]
\end{lem}

\begin{proof}
  Define $\delta_X = (v_X, \mathbf{I})$, where \begin{align*}
    v_X : \bars{\Box X} &\longrightarrow \bars{\Box^2 X} \\
	  (x, a)        &\longmapsto ((x, a), a)
  \end{align*} If $a \in \dbars{x}_X$, then $\mathbf{I} \cdot a
  \simeq a \in \{a\} = \dbars{((x, a), a)}_{\Box^2 X}$, so
  $\mathbf{I}$ indeed tracks $v_X$. To show naturality for a given
  arrow $(f, r) : X \rightarrow Y$, we chase around the diagram: \[
    \begin{tikzcd}
      (x, a)
	\arrow[r, mapsto, "f_r"]
	\arrow[d, mapsto, swap, "v_X"]
      & (f(x), r \cdot a)
	\arrow[d, mapsto, "v_Y"] \\
      ((x, a), a) 
	\arrow[r, mapsto, swap, "\left(f_r\right)_r"]
      & \left((f(x), r \cdot a), r \cdot a\right)
    \end{tikzcd}
  \] and so the diagram commutes up to $\sim$.  Note that the
  tracking elements along the composites are respectively
  $\mathbf{B} \cdot \mathbf{I} \cdot r$ and $\mathbf{B} \cdot r
  \cdot \mathbf{I}$.
\end{proof}

The components of $\delta : \Box \natexp{} \Box^2$ actually
satisfy our special property:

\begin{lem}
  Each component of $\delta : \Box \natexp{} \Box^2$ is a
  reasonable quoting device.
\end{lem}

\begin{proof}
  Given any $(a, r) : \mathbf{1} \rightarrow \Box X$, we chase around
  the diagram, where $n_0$ is the function component of $m_0$: \[
    \begin{tikzcd}
      \ast
	\arrow[r, mapsto, "a"]
	\arrow[d, mapsto, swap, "n_0"]
      & (a(\ast), r \cdot \overline{0})
	\arrow[d, mapsto, "v_X"] \\
      (\ast, \overline{0})
	\arrow[r, mapsto, swap, "a_r"]
      & \left((a(\ast), r \cdot \overline{0}), r \cdot \overline{0} \right)
    \end{tikzcd}
  \]
\end{proof}

Hence, we can put everything together to prove that 
\begin{thm}
  $(\Box, \epsilon, \delta)$ is a comonadic exposure.
\end{thm}

\begin{proof}
  It suffices to verify the coherence conditions.  Regarding the
  first one: \[
    \begin{tikzcd}
      (x, a)
	\arrow[r, mapsto, "v_X"]
	\arrow[d, mapsto, "v_X", swap]
      & ((x, a), a)
	\arrow[d, mapsto, "v_{\Box X}"] \\
      \left((x, a), a \right)
	\arrow[r, mapsto, "\left(v_X\right)_{\mathbf{I}}", swap]
      & (((x, a), a), \mathbf{I} \cdot a) = (((x, a), a), a)
    \end{tikzcd}
  \] which commutes, since $\mathbf{I} \cdot a \simeq
  a$. Both the tracking elements along each composite are $\mathbf{B}
  \cdot \mathbf{I} \cdot \mathbf{I}$, so the diagram actually
  commutes on the nose. Regarding the second one: \[
    \begin{tikzcd}
      (x, a)
	\arrow[r, mapsto, "v_X"]
	\arrow[d, mapsto, "v_X", swap]
	\arrow[rd, mapsto, equal]
      & ((x, a), a)
	\arrow[d, mapsto, "u_{\Box X}"] \\
      \left((x, a), a \right)
	\arrow[r, mapsto, "\left(u_X\right)_{\mathbf{I}}", swap]
      & (x, \mathbf{I} \cdot a) = (x, a)
    \end{tikzcd}
  \] which commutes, since $\mathbf{I} \cdot a \simeq
  a$. Once more, both tracking elements are $\mathbf{B} \cdot
  \mathbf{I} \cdot \mathbf{I}$, so commutation is again on the nose.
\end{proof}


